Validated Strong Consensus Protocol for Asynchronous Vote-based Blockchains

Vote-based blockchains construct a state machine replication (SMR) system among participating nodes, using Byzantine Fault Tolerance (BFT) consensus protocols to transition from one state to another. Currently, they rely on either synchronous or partially synchronous networks with leader-based coordination or costly Asynchronous Common Subset (ACS) protocols in asynchronous settings, making them impractical for large-scale asynchronous applications. To make Asynchronous SMR scalable, this paper proposes a \emph{validated strong} BFT consensus model that allows leader-based coordination in asynchronous settings. Our BFT consensus model offers the same level of tolerance as binary byzantine agreement but does not demand consistency among honest nodes before they vote. An SMR using our model allows nodes to operate in different, tentative, but mutually exclusive states until they eventually converge on the same state. We propose an asynchronous BFT protocol for vote-based blockchains employing our consensus model to address several critical challenges: how to ensure that nodes eventually converge on the same state across voting rounds, how to assure that a blockchain will steadily progress through epochs while reaching consensus for previous epochs, and how to maintain robust byzantine fault tolerance. Our protocol greatly reduces message complexity and is the first one to achieve linear view changes without relying on threshold signatures. We prove that an asynchronous blockchain built on our protocol can operate with the \emph{same} simplicity and efficiency as partially synchronous blockchains built on, e.g. HotStuff-2. This facilitates deploying asynchronous blockchains across large-scale networks.

==> main-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}\textbf {Assumption: }We assume the existence of a robust adversarial model and compliance-checking mechanisms as described in Sec.~\ref {4.4.1}, particularly focusing on filtering non-compliant votes. \par \textit {Step 1: Assume for Contradiction} \par Assume that the lemma is false. That is, assume there exists an adversarial node \( j \) whose vote \( V_j^{(k)} \) for a block stemming from \( B_{k'} \) at height \( k \) is linked by an honest node at height \( k+1 \), even though \( B_{k'} \) is not stem from the most supported branch according to \( \operatorname {VC}_j^{(k)} \). \par \textit {Step 2: Adversarial Vote Analysis} \par Under the voting rules, a compliant vote is only linked to a vote if it satisfies the criteria outlined for a compliant vote. According to the criteria, a node \( i \) will only consider \( V_j^{(k)} \) if: - The block \( B_{k'} \) voted on by \( j \) has the highest vote count among all blocks at height \( k' \) of the same branch and this branch stems from the most supported branch, according to \( \operatorname {VC}_j^{(k)} \). \par \textit {Step 3: Invoking the Voting Rule and Mechanisms} \par Given that \( V_j^{(k)} \) was linked by an honest node \( i \) at height \( k+1 \), it implies that: \par \begin {itemize} \item \( V_j^{(k)} \) adhered to the honest voting criteria~\ref {p2}, contradicting the assumption that \( B_{k'} \) was not the root of the most supported branch stemming from the most supported branch according to \( \operatorname {VC}_j^{(k)} \) . \item Therefore, if \( B_{k'} \) was indeed not the root of the most supported branch stemming from the most supported branch based on \( \operatorname {VC}_j^{(k)} \), the honest nodes would have disregarded \( V_j^{(k)} \) due to the enforcement of compliance checks \( \operatorname {VC}_j^{(k)}[B_{k'}] < \operatorname {VC}_j^{(k)}[B'_{k'}] \) for any other block \( B'_{k'} \) with higher support. \end {itemize} \par \textit {Step 4: Security Reduction} \par By reduction, if \( V_j^{(k)} \) were accepted and linked by an honest node without \( B_{k'} \) being the root of the most supported branch stemming from the most supported branch, it would imply that the voting mechanism failed to correctly enforce its rules or detect non-compliance. This failure would represent a breakdown in the integrity of the voting process, directly contradicting the protocol's assumption of reliable, compliant vote counting and validation mechanisms. \par \textbf {Conclusion}: Given the system's design to filter non-compliant votes and enforce the honest model, it is contradictory to assume a scenario where an adversarial vote for a less supported branch gets linked by an honest node. So, by contradiction, the lemma holds under the protocol's operational assumptions and security model. Thus, a Byzantine node must vote for the most supported branch to their local knowledge to have their vote considered by others.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}\textbf {Assumption:} Assume that our protocol correctly implements and enforces the rules stated in the consensus mechanism, especially the handling of node votes, double-voting detection, and compliance with voting rules according to vote counts. \par \textit {Step 1: Assume for Contradiction} \par Assume, for the sake of contradiction, that there exists another block \( B''_{k'} \) different from \( B_{k'} \), which is also accepted in consensus at the same height \( k' \), despite \( B_{k'} \) having been accepted following the consensus criteria. \par \textit {Step 2: Analysis of the Consensus Criteria} \par Under the consensus rules: \begin {enumerate} \item All nodes in a subset \( NG \) of size at least \( N-f \) (where \( f \) is the number of possible faulty nodes) have voted for \( B_{k'} \) such that: \[ \operatorname {VC}_{j}^{(k)}[B_{k'}] - t > \operatorname {VC}_{j}^{(k)}[B'_{k'}(j)] + \operatorname {VC}_{j}^{(k)}[U_{k}] - \operatorname {VC}_{j}^{(k)}[U_{k'}] - 1 \] where \( t \) accounts for potential double-voting between \( k' \) and \( k-1 \). \item The condition essentially states that the support for \( B_{k'} \) exceeds any potential support for any other block, taking into account uncounted votes and potential double votes. \end {enumerate} \par \textit {Step 3: Security Reduction} \begin {itemize} \item By the consensus condition, for \( B_{k'} \) to be accepted, it must be the most supported block at height \( k' \) after considering all compliant votes. \item If \( B''_{k'} \) were also accepted under these conditions, it would imply that \( B''_{k'} \) too met the threshold in Eq. (\ref {acc7}), contradicting our initial validation that \( B_{k'} \) had decisively more support. \item Such a scenario would suggest that the system has either failed to detect and discard invalid or non-compliant votes (such as those involved in double-voting) or has incorrectly calculated the vote totals. This would violate the integrity of the voting mechanism designed to prevent exactly such an occurrence. \end {itemize} \par \textit {Step 4: Implication of the Assumption Being False} \par \begin {itemize} \item If the lemma were false, it would imply that the system’s core security features (accurate vote counting, compliant vote validation, and correct execution of consensus protocol) are flawed. \item Since the protocol relies on these features to ensure network security and integrity, which are assumed to be reliable, the assumption that two different blocks can be accepted at the same height must be false. \end {itemize} \par \textbf {Conclusion:} The acceptance of two different blocks \( B_{k'} \) and \( B''_{k'} \) in the same consensus height would directly contradict the enforcement of the voting and consensus rules. Therefore, by security reduction, if our security mechanisms are functioning as intended, no such scenario can occur. Hence, the lemma holds under the conditions set by our protocol, ensuring the uniqueness of the accepted block at any consensus height.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}We model the process of convergence as a discrete-time Markov chain (DTMC) with state space $\{1, 2, \dots , m\}$, where each state $x_r = x$ represents the number of distinct input values remaining at round $r$. The absorbing state is $x = 1$, where consensus is reached, and no further transitions occur. \par \textbf {State Space and Transitions:} \begin {itemize} \item The process begins at state $x_r = m$, where all $m$ distinct input values are still in play. \item The system transitions between states based on whether one or more input values are eliminated in each round. A transition from $x_r = x$ to $x_{r+1} = x-j$ represents the elimination of $j$ input values in that round, where $j \in \{1, 2, \dots , x-1\}$. \item The absorbing state is $x = 1$, where all nodes vote for the same input value and convergence is reached. \end {itemize} \par \textbf {Transition Probabilities:} Let $P(x \to x)$ be the probability that no progress is made in a round, meaning no input value is eliminated. Let $P(x \to x-j)$ be the probability that $j$ input values are eliminated in a round. \par \begin {enumerate} \item \textbf {No Progress Probability $P(x \to x)$}: This occurs when the nodes \emph {nearly equal supporting the remaining $x$ input values}, and no clear majority emerges. The probability of no progress is higher when the votes are more evenly distributed. Based on binomial distribution approximations, \emph {a very lost upper bound} probability can be written as: \[ P(x \to x) \approx \frac {1}{\sqrt {2 \pi \frac {N-f}{4}}} \] The rational behind this probability is that consider the case where there are two equally supported branches rooted by block $A$ and $B$, and each has $\frac {N}{2}$ votes. Each node samples $N-f$ votes from this set. Afterwards, the probability that exactly $\frac {N}{2}$ nodes vote for each branch (thus no change in the poll) can be approximated using the \textit {binomial distribution}: \[p(o) = \binom {N-f}{o} \left ( \frac {1}{2} \right )^o \left ( \frac {1}{2} \right )^{(N-f-o)} = \binom {N-f}{o} \left ( \frac {1}{2} \right )^{N-f}\]where $o = \frac {N-f}{2}$. The probability (very loose upper bound) is thus approximately:$p_{(\text {no progress})} \approx \frac {1}{\sqrt {2 \pi \frac {N-f}{4}}}$. \par \item \textbf {Progress Probability $P(x \to x-j)$}: The probability that $j$ input values are eliminated in the round depends on how biased the vote distribution is. As $x$ decreases (fewer input values remain), the likelihood of eliminating multiple input values at once increases if the vote distribution skews towards one or more dominant input values. \par The probabilities for eliminating $j$ input values in a single round can be modeled as a decreasing geometric-like distribution where the probability of eliminating more input values declines as $j$ increases: \[ P(x \to x-j) = \alpha _j \cdot P(\text {progress}), \quad \sum _{j=1}^{x-1} \alpha _j = 1 \] where $\alpha _j$ is a weight assigned to the probability of eliminating $j$ input values. For simplicity, these weights can reflect the natural tendency that eliminating fewer input values is more likely than eliminating more in each round. \end {enumerate} \par \textbf {Transition Matrix:} The transition matrix $P$ for this Markov chain is defined as follows, where $P_{ij}$ represents the probability of transitioning from state $i$ to state $j$: \[ \small P = \begin {pmatrix} 1 & 0 & 0 & \dots & 0 & 0 \\ P(2 \to 1) & P(2 \to 2) & 0 & \dots & 0 & 0 \\ P(3 \to 1) & P(3 \to 2) & P(3 \to 3) & \dots & 0 & 0 \\ \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\ P(m \to 1) & P(m \to 2) & P(m \to 3) & \dots & P(m \to m-1) & P(m \to m) \\ \end {pmatrix} \] \par \textbf {Expected Time to Absorption:} The goal is to calculate the expected time to reach the absorbing state $x = 1$, starting from state $x = m$. Let $t_x$ represent the expected number of rounds to reach state $x = 1$ starting from state $x$. The recurrence relation for $t_x$ is: \par \[ t_x = \frac {P(x \to x) + \sum _{j=1}^{x-1} P(x \to x-j) + \sum _{j=1}^{x-1} P(x \to x-j) \cdot t_{x-j}}{1 - P(x \to x)} \] \par This equation indicates that the expected time $t_x$ depends on either staying in the same state (with probability $P(x \to x)$) or transitioning to lower states, reducing multiple input values at once. The summation term accounts for all possible transitions, where $j$ input values are eliminated in a round. \par Rearranging the terms: \par \[ t_x = \frac {1 + \sum _{j=1}^{x-1} P(x \to x-j) \cdot t_{x-j}}{P(\text {progress})} \] \par By solving this recurrence relation starting from $t_1 = 0$ (the absorbing state), we can calculate the expected time to convergence. \par \textbf {Worst-Case Convergence Time:} In the worst case, when the votes are nearly uniformly distributed, $P(x \to x)$ remains high, and progress is slow. The recurrence relation shows that when $P(x \to x)$ is significant, the expected time $t_x$ increases linearly with $x$, leading to an overall convergence time of $O(m)$. \par \textbf {Amortized Case Convergence Time:} In the average case, as $x$ decreases, the vote distribution becomes less uniform, and the probability of eliminating multiple input values in a round increases. Once a majority input value emerges, recursive vote linking amplifies its support, leading to exponential convergence. The expected time to consensus in this case is $O(\log m)$. \par \end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Assume that all $m$ blocks receive $\frac {N}{m}$ votes at the first voting height. Ideally, each node recognizes multiple blocks as equally supported; subsequently, each node votes randomly. The least-supported blocks will be discarded, reducing $m$. However, nodes only have access to partial voting history, which could result in divergent perspectives. For example, in an $N=12, f=3$ system with $m=4$ blocks ($A, B, C, D$), when the global view of votes is $AAABBBCCCDDD$, nodes might hold different local views such as $AAABBCCDD$ and $BBBAACCDD$, depending on the first $N-f$ compliant votes they receive. If the adversary controls the set of votes received by the honest nodes, it can manipulate them to consistently vote for the same branch by carefully selecting which $N-f$ votes they receive first. This attack can prevent the reduction of $m$, thus hindering liveness.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}\noindent \textbf {Safety of the established consensus:} Though a node may oscillate between different blocks, this inconsistency will not affect the already accepted blocks because if $B_{k'}$ is already accepted before or at $k$, $\operatorname {VC}_{i}^{(k)}[B_{k'}] \leq \operatorname {VC}_{i}^{(k)}[B'_{k'}(i)] + \operatorname {VC}_{i}^{(k)}[U_{k}] - \operatorname {VC}_{i}^{(k)}[U_{k'}]$ will not occur. \par \noindent \textbf {Safety of adversary controlling the delays:} An adversary may control which $N-f$ votes are received by each honest node and can trigger indication of potential loss of liveness. However, the strong common coin is flipped later. Thus, the adversary cannot influence the random vote decisions. \par \noindent \textbf {Liveness:} The randomness of voting that assists in breaking away from the loss of liveness can be provided by a local coin. However, allowing not voting for the most supported branch enables a strong adaptive adversary to escape from the irreversible convergence enforced by the vote graph if it can observe the votes of others before casting its own. By implementing a strong common coin, the adversary must follow the unpredictable coin value. This provides an unbiased randomness necessary to ensure liveness. \par If fewer than $N-f$ nodes participate in the coin flip, the coin flip will not be generated. There must exist some honest node $i$, where the most supported branch $B$ satisfies the condition $\operatorname {VC}_i^{(k)}[B] > \operatorname {VC}_i^{(k)}[B'] + \operatorname {VC}_i^{(k)}[U_k] - \operatorname {VC}_i^{(k)}[U_{k'}]$ for any other branch $B'$. In this case, node $i$ will vote for branch $B$ at height $k$ instead of participating in the coin flip. Then, the other honest nodes will eventually receive $V_i^{(k)}$ according to the assumption that the adversary cannot delay messages indefinitely. They can then link their votes to a different set of $N-f$ votes from the previous height and vote for the most supported branch to their knowledge after acquire the missing votes from $G_i^{(k)}$.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}There are two cases, which we analyze separately below: \par Case A (practical liveness, the adversary does not control the delays of at least $N-f$ nodes): Because each node receives a random set of $N-f$ votes, it can be seen as flipping a weak random coin, as discussed in Sec.~\ref {4.6.1}. This will monotonically reduce the input values until only one remains. \par Case B (The adversary constantly controls the delays of at least $N-f$ nodes): If the condition $\operatorname {VC}_j^{(k-1)}[B_{k'}(j)] < \operatorname {VC}_j^{(k-1)}[B'_{k'}(j)] + \operatorname {VC}_j^{(k-1)}[U_k] - \operatorname {VC}_j^{(k-1)}[U_{k'}]$ is uniformly satisfied by at least $N-f$ votes from height $k-1$ cast by any node $j$, and $k-k'>log_2 (N)$, indicating potential for multiple supported branches (as detailed in Sec.~\ref {4.6.2}), honest nodes initiate a coin flip. The coin flip is a strong common coin mechanism that produces a common random value that cannot be influenced by the adversary once initiated. The outcome of the coin flip dictates which branch the honest nodes will vote for at height $k$, providing a way to break the tie uniformly across all honest nodes. Since the adversary cannot predict or manipulate the outcome of the coin flip once it is triggered, the coin flip ensures that, after each round, the chance of all honest nodes aligning on the same branch increases as it can be seen as the nodes receiving a random set of $N-f$ votes of the last height, akin to Case A. \par Therefore, the eventual convergence is guaranteed.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We first assume all nodes adhere to the voting rules defined in Sec.~\ref {lba}. Thm.~\ref {thm:liveness} shows that they will converge to the same branch despite the presence of strong adaptive adversary. After this process, Eq.~\ref {acc7} will be achieved. The convergence and exclusivity of the votes guarantee irreversible block acceptance, as suggested in Lem.~\ref {k2-new}. \par Now, consider what happens if violating the voting rules: \par \begin {itemize} \item \textbf {Non-compliant votes:} Lem.~\ref {k1} proves that any non-compliant vote, i.e., those exhibiting characteristic (C2) of adversarial behavior, is disregarded by honest nodes upon receiving them. \par \item \textbf {Double voting:} Concerning double voting (adversarial characteristic (C1) and a breach of honest model~\ref {p1}), Lem.~\ref {k2-new} proves that the criteria for block acceptance already consider and mitigate the effects of double voting. Eq.~\ref {acc7} suggests the system's ability to achieve consensus despite double voting. \end {itemize} \par Hence, non-compliant votes and double voting do not influence the outcome. If the liveness of consensus-derivation is secured, agreement and termination are assured.\end{proof}

